Finding Crash-Consistency Bugs with Bounded Black-Box Crash Testing

We present a new approach to testing file-system crash consistency: bounded black-box crash testing (B3). B3 tests the file system in a black-box manner using workloads of file-system operations. Since the space of possible workloads is infinite, B3 bounds this space based on parameters such as the number of file-system operations or which operations to include, and exhaustively generates workloads within this bounded space. Each workload is tested on the target file system by simulating power-loss crashes while the workload is being executed, and checking if the file system recovers to a correct state after each crash. B3 builds upon insights derived from our study of crash-consistency bugs reported in Linux file systems in the last five years. We observed that most reported bugs can be reproduced using small workloads of three or fewer file-system operations on a newly-created file system, and that all reported bugs result from crashes after fsync() related system calls. We build two tools, CrashMonkey and ACE, to demonstrate the effectiveness of this approach. Our tools are able to find 24 out of the 26 crash-consistency bugs reported in the last five years. Our tools also revealed 10 new crash-consistency bugs in widely-used, mature Linux file systems, seven of which existed in the kernel since 2014. Our tools also found a crash-consistency bug in a verified file system, FSCQ. The new bugs result in severe consequences like broken rename atomicity and loss of persisted files.

==> abstract-old.tex <==
\begin{abstract}
We present \sysname, a set of tools to systematically find
crash-consistency bugs in Linux file systems. \sysname automatically
constructs different workloads to test whether the target file system
recovers correctly after crashes at different points. \sysname
exploits two insights. First, we observe that crash consistency only
depends upon the file system and the storage state at the point of the
crash; \sysname thus \emph{constructs} possible crash states for a
given workload, mounts the file system on each crash state, and checks
for crash consistency. Second, we observe that crash-consistency bugs
reported in the wild do not require large workloads containing many
file-system system calls to reproduce bugs; thus, \sysname
exhaustively explores all workloads of small sizes to find bugs. Based
on this strategy, we have been able to reproduce 14 previously
reported crash-consistency bugs in btrfs, ext4, and F2FS. We have also
found three new bugs in ext4, btrfs, and F2FS which have been
acknowledged and patched. A different research group is currently
using \sysname to test the crash consistency of their new research
file system.
\end{abstract}


==> abstract-old2.tex <==
\begin{abstract}
A system is crash consistent if it recovers to a correct state after a
crash due to power loss or kernel panic. We present \sysname, a tool
to automatically find crash-consistency bugs in Linux file
systems. \sysname works by profiling a given workload, and
constructing different crash states that are possible if the system
had crashed at different points during the workload. Unlike existing
tools for testing crash consistency, which require the developer to
explicitly write workloads and checkers, \sysname takes the human out
of the loop; \sysname systematically constructs and checks different
workloads based on the maximum number of file-system system calls
possible in the workload. \sysname leverages the fact that revealing
crash-consistency bugs does not require long and complex workloads;
simple workloads are enough, if the workloads are constructed
systematically. With systematically constructed workloads of small
sizes, \sysname reproduces \emph{all} previously reported
crash-consistency bugs in ext4, btrfs, and F2FS. \sysname also found
three new bugs in btrfs and F2FS, which have been acknowledged and
patched.
\end{abstract}


==> abstract-old3.tex <==
\begin{abstract}
We present \sysname, a fully automatic system to systematically test
whether file systems recover correctly after a crash. There are two
major components in \sysname: a crash-state generator which generates
possible states after a crash for a given workload, and a workload
generator which automatically generates all workloads of a given
length to run on the target file system. By interposing on system
calls in the workload, \sysname maintains enough information to
automatically check what the correct state should be after recovery
from the crash. \sysname takes advantage of two insights obtained from
our study of crash-consistency bugs reported in the last five years:
first, all reported crash-consistency bugs require only small
workloads (up-to four main file-system operations) to be revealed on a
crash; second, it is sufficient to crash after persistence-related
system calls like \sysfsync to reveal bugs. \sysname combines these
two insights to exhaustively generate and check small workloads for
our target file systems. By exhaustively checking 1.5 million
workloads of length four or less, \sysname is able to find 27 out of
the 29 crash-consistency bugs reported in the last five
years. \sysname also revealed three \emph{new} crash-consistency bugs
in widely used Linux file systems that lead to file-system corruption,
two of which have already been fixed in the Linux kernel. The utility
and ease-of-use of \sysname is indicated by another international
research group already using \sysname to test their research file
system.
\end{abstract}


==> case.tex <==
\section{Studying Crash-Consistency Bugs}
\label{sec-study}

We present an analysis of crash-consistency bugs reported in four
Linux file systems (ext4, btrfs, xfs, F2FS) over the past five years
(since 2013). We collected these bugs from two sources; first, we look
at the mailing lists to find reports of crash-consistency bugs;
second, we also examine \xfstests test cases that were added in
response to a crash-consistency bug report.

Overall, there are 30 bugs spread across the four file systems. Among
these file systems, ext4 and xfs are the most mature, having undergone
more than 15 years of active development. As a consequence, these file
systems have few crash-consistency bugs reported. btrfs and F2FS are
new file systems, having been introduced only in 2009 and 2012. btrfs in
particular seeks to provide a lot of complex features such as snapshot, cloning, out-of-band deduplication and compression.

btrfs is a copy-on-write filesystem, that manages all its metadata in various B+ trees emerging from 
the Tree of Tree roots. Inodes, bitmaps, directory entries, extent info etc are all an item in a copy-on 
write B+ tree. This makes achieving crash consistency tricky, as the updates have to be propagated to 
several trees. 

Analyzing crash consistency bugs over the past 5 years reveals how crash consistency has evolved in 
btrfs.

\vheading{Fsync and the btrfs replay log (3.13 kernel)}

In btrfs, a persisted inode/directory entry goes into the filesystem (subvolume) tree, and on fsync, the 
changes are written to the fsync log. Several of the bugs revealed in Linux kernel 3.13 arise due the 
conflicts in updating the metadata across the FS tree and the fsync log.  Suppose we create a file foo 
and sync it. This ensures the directory entry for file foo is present in the FS tree. We  then create a 
new sibling to the file foo and fsync the parent directory. If we crashed now, during log replay, the 
directory inode's i\_size is calculated by summing up the size of dentries of the new sibling, and the 
previously persisted file foo. This lead to an incorrect i\_size of the directory inode, as the dentry foo 
was accounted for twice during log replay. As an effect, even if the file foo and its sibling is removed, 
the directory i\_size remains non zero and hence becomes unremovable~\cite{btrfs-generic34}.

Another scenario where the fsync log replay code incorrectly updated the directory i\_size, was when 
the filesystem crashed soon after removing a hard link to a file, and fsync-ing the file. In this case, the 
log replay did not decrement the i\_size of the parent directory due to the unlink of a file, but the dentry 
is removed. Therefore, the directory was unremovable, even after deleting all the entries within~\cite{btrfs-generic39}.

While these bugs in the recovery logic that incorrectly accounted for the directory i\_size to be larger 
than original were fixed, btrfs soon discovered a new class of bugs where the recovery logic ended up 
leaving around stale handles to persisted files that made the files inaccessible and unremovable. 

Consider a workload where a hard link is added to an existing file
foo. The dentry of foo exists in the FS tree, while the newly added
link is in the fsync log. During replay, the link count of file foo
remains un updated, while the newly added hard link dentry was still
visible. This resulted in a stale file handle while referencing the
link-file, and making it impossible to be accesses or removed. Because
of this, the directory containing these files was also
unremovable~\cite{btrfs-generic-unremovable}.  Btrfs fixed this issue
in the direct path - i.e. the case where there was an explicit \fsync
on the file or its parent directory, they ensured that link count is
updated correctly whenever the directory entry is persisted. However
soon btrfs encountered the same problem through a different code
path. If a hard link is created to a file, but some other operation in
the same directory inadvertently persists the link- file, we would
again see a directory entry for the link-file, but the original file's
link count remains unupdated. THe developers acknowledge that this was
not a regression, or a new issue due to the previous fix, but existed
in the kernel ever since log tree was added~\cite{btrfs-generic104}.
However, it took 4 months to track down that a known bug could be
triggered through an alternate code path. The previous workload
required creating hard links and fsyncing the original file/parent
directory, while this one requires that we \fsync a sibling in the
same directory. A systematic workload generation approach would have
been able to identify both the above bugs at the same time.

While all these bugs hint at btrfs crash consistency mechanisms and replay logic to be naive, fast 
forward a few linux kernel versions, btrfs had a different category of crash consistency bugs.

\vheading{Rename and the btrfs replay log (4.4 kernel)}

The 3.1x kernels were traumatized by the interaction of link system call with the btrfs replay logic and 
in the 4.x kernels, it was the turn of rename. Suppose a file(directory) A is renamed to B and a new 
file(directory) is created with the old name (A) of the renamed file(directory). If the file A is fsynced and  
crashed, the recovery logic ended up completely removing file B, and if B was a directory, all its 
contents were also lost~\cite{btrfs-generic341}.

Contrary to this workload, if we move a file(directory) to a new parent, and only \fsync the new parent, 
then the file(directory) was persisted in the new parent, but at the same time, not removed from the old 
parent. This not just makes the rename system call non atomic at storage, but also leaves stale 
handles to the file in the old parent directory, thereby making it unremovable~\cite{btrfs-generic343}.

\vheading{Today's scenario : File system unmountable (4.15 kernel)}
The nature of btrfs crash consistency bugs has only gotten more serious over the years. From losing 
files, to leaving around stale file handles - the severity of the bugs have reached the point where the 
filesystem becomes unmountable after a crash due to a failed log replay. Consider a scenario where 
we remove a hard link from a file , and create a new file in the same directory with the name of the 
removed link. The fsync log while processing the reference to the removed inode, updates the FS tree  
to reflect the decremented link count,  leaving a dangling directory index key in the parent. On 
processing the next entry in the replay log, since the same name is reused and the directory index still 
exists, the replay logic tries to unlink the file again, which fails. This makes the filesystem 
unmountable, unless the replay log is wiped off~\cite{btrfs-generic-link-unlink}

A complicated workload is not essential to result in a crash consistency bug. Take F2FS for example. 
While allocating blocks beyond the end of the file using fallocate(with the KEEP\_SIZE flag), if we 
fdatasync the file and then crash, on recovery the file recovers to an incorrect size. The KEEP\_SIZE 
flag must ensure that the blocks beyond eof are allocated, but the file size remains unchanged. 
However, F2FS fails to log the unchanged filesize on fdatasync, and thereby recovers the filesize based 
on the value of last allocated block. F2FS fixed this bug in the case of fallocate system call~\cite{f2fs-generic392}. However, fallocate system call 
itself has several options like ZERO\_RANGE,  PUNCH\_HOLE, INSERT\_RANGE etc, and 
developers fail to systematically test a bug with all possible parameter options of the system call.  
\sysname identified another possible codepath where the same bug would reproduce itself and it was 
patched recently.

\vheading{Inferences from crash consistency bugs over the years}
\begin{enumerate}
\item Interaction between multiple log trees is one of the main reasons that result in crash consistency 
bugs.
\item The workloads to reproduce these bugs are simple - typically less than 5 system calls
\item Bugs with the same root cause have been identified and reported several months apart - 
systematic testing of workloads would have identified correlated bugs much faster.

\end{enumerate}




==> cm.tex <==
\section{\sysnamet Infrastructure}
\label{sec-infra}

%\input{fig-arch}

\vheading{Challenges in Testing Crash Consistency}. Despite the conceptual
simplicity of the problem, efficiently testing for file system crash consistency
is non-trivial. A myriad of variables like the current load on the system,
memory usage, size of write requests, block device drivers, and physical devices
can all contribute to crash consistency bugs. However, picking apart this mess
of variables to determine whether or not the file system itself is crash
consistent for any fixed set of variables is exceptionally hard. This problem is
further complicated by the fact that file system crash consistency behavior
differs between file systems, and is often not thoroughly documented. All of
this combined means that the real behavior for individual file systems can
sometimes only be discovered by talking to file-system developers or empirically
exploring the crash consistency behavior of the file system.

\am{can we get a citation on that mailing list thread talking about how POSIX is
broken and how hard it is to create standardized documentation on file systems?}

\vheading{Goals}.
\lsysname is responsible for providing a host of features that make logging
information about file system workloads, generating crash states, and
automatically testing the generated crash states efficient. As all of these
functions are disjoint, \lsysname can be broken down into three distinct parts:
a logging system that collects information about a given file system workload
while it runs, a crash state generator, and an auto checker that determines if
the file system in the generated crash state maintains its crash consistency
guarantees. The goal of the logging system is to provide sufficient information
for the crash state generator and the auto checker to reproduce a vaild crash
state or verify that a crash state is consistent. The crash state generator
focuses on outputting a series of disk writes that could occur when a computer
crashes in the middle of updating the file system. Finally, the auto checker
aims to provide fast and efficient tests for crash states generated immediately
after a persistence point.

\am{Writing this, I get the feeling that this section would fit better after the
part about generating crash states simply because then I could reference terms
that are defined in that section. Also, Vijay, please read this over as I am not
sure I discussed the content that you were really interested in in the Cache
Model section}

\vheading{Cache Model}.
\lsysname seeks to emulate a system that has the Linux storage stack described
in \sref{sec-mot}, paired with a storage device that has an onboard cache which
buffers data internally. Two key insights allow \lsysname to
emulate this cache model with subsets of disk operations in the target epoch.
The crash state generator only needs to consider subsets of operations because
permutations of the operations in the final epoch could lead to incorrect disk
behavior. Consider the two cases for operations in the target epoch: either all
the operations are disjoint and affect different portions of the storage device
or there are some operations that overlap. For the case where the operations are
disjoint, it is easy to see that any permutation of a subset of these operations
will lead to an equivalent crash state. For subsets of operations that overlap,
permutations can lead to incorrect behavior. For example, given two overlapping
operations A and B, where operation A is issued and marked completed (but not
necessarily persisted) before B, if one were to permute the operations such that
B came before A, it could result in a sort of "time travel" for the issue order
of the operations. On a real storage device, if operation A were present in the
device cache when operation B were issued, the cache would simply replace
operation A with operation B. Therefore, simply picking an ordered subset of the
operations recorded in the target epoch suffices to generate valid crash states.

\vheading{Profiling Workloads}. The profiling code in \lsysname tracks three
different things during workload execution. First, it tracks the system calls
that the workload makes at the user level. Next, it tracks information about
disk requests at the block device layer. Finally, it creates lightweight
snapshots at every persistence point in the workload. At the highest level,
\lsysname interposes on the system calls that the workload makes to the kernel.
By tracking these system calls, \lsysname can construct a high level view of
what the workload is doing, allowing it to better track which file should be
tested after a persistence point in the generated crash state. \lsysname
accomplishes this tracking by providing a set of wrapper functions for system
calls. Since workloads are automatically generated by \usysname, it is trivial
for \usysname to swap a call to the \syswrite function out for a
\lsysname-specific write function. The wrappers that \lsysname provides tracks
information like the path of the file being operated on, the data range being
changed, and, for syscalls that write data, the actual data being written.
\lsysname also provides a special \chkpt function which the user can call after
any persistence operation. The \chkpt function places a mark both in the series
of recorded system calls as well as the series of recorded block device
operations. Since the \chkpt call is synchronous while much of the Linux storage
stack is asynchronous, \chkpt calls are only supported immediately after a call
like \sysfsync which creates a persistence point.

At a much lower level, \lsysname provides a wrapper block device capable of
recording all requests sent to it. This wrapper device is compiled into a kernel
module which can be inserted into the host machine's kernel at runtime,
therefore avoiding the need for lengthy kernel recompiles. The wrapper device
works by inspecting all requests sent to it and recording the data, size, disk
sector, and flags for write, \flagfua, and \flagflush  requests. \lsysname is
not required to record the read requests because they do not have the potential
to change the layout of data on the storage device. Therefore, the subset of
requests it does record is sufficient to to faithfully reconstruct a series of
changes made to the disk during the workload. After profiling, the recorded
information is exported to user space via an \sysioctl call so it can be
manipulated by the crash state generator.

\lsysname also provides a block device that allows the system to make snapshots
of the file system in the workload. Each time a workload is run in \lsysname,
the system executes the workload until successive \chkpt operations. At each
\chkpt, \lsysname takes a snapshot of the current disk state so that the auto
checker has a oracle disk image to which it can compare the contents of crash
states. Once the snapshot is created, \lsysname restarts the workload so that it
can reach the next \chkpt operation. This process continues untill the entire
workload has executed. Even though this process may seem a little cumbersome,
the workloads generated by \usysname are small, typically no more than five file
system operations in length, with one or two persistence points in the workload.
Thus, running the workload multiple times does not greatly affect the runtime of
\lsysname.

\am{What is the maximum number of *sync operations that can be in workload? The
preceeding pargraph has a reference to that}

\vheading{Constructing Crash States}. \lsysname has two modes for construcitng
crash states. The first mode sequentially replays the workload to each
successive mark made by the \chkpt function and then tests the resulting disk
image. The second mode of operation constructs crash states from a subset of the
recorded disk operations. Sequentially replaying disk operations and checking
for file system consistency at every mark made by \chkpt focuses testing efforts
on the persistence points of the workload. The algorithm in the crash state
generator for this mode is simple: it just traverses the list of logged disk
operations until it finds a \chkpt mark. At each mark, it generates a crash
state with the disk operations until that mark.

The goal of the algorithms responsible for constructing crash states
is to simulate reordering, merging, and buffering of IO requests that could take
place in the Linux storage stack and the storage device's cache. Conceptually,
the series of disk operations recorded during the profiling stage of \lsysname
can be thought of as a series of \cmepochs, each of which is terminated by an
operation containing a \flagflush or \flagfua flag.

Assuming a storage device understands and adheres to the semantics of the
\flagflush and \flagfua flags, a crash state can be generated by splitting it
into two parts: the \cmepochprefix and the \cmepochtarget that the "crash"
occurs in. The epoch prefix is the set of complete epochs that are persisted
on disk prior to the crash while the target epoch is the partially persisted
epoch in which the crash occurs. Therefore, a simple algorithm for generating
crash states can be divided into two steps: 1) randomly picking an epoch prefix
for the current crash state and 2) randomly dropping a subset of the write
requests in the target epoch. The first step is responsible for determining
where in the workload the crash occurs since it determines how much data is
already completely persisted in the crash state. The second step emulates the
Linux storage stack and storage device cache by making it appear as if only some
of the operations in the target epoch were persisted (\ie the storage device
wrote them to disk) while others were dropped (\ie the storage device had these
operations stored in its volatile cache when the crash occurred).

Since the size of the write operations the kernel issues to a storage device can
be multiple pages of data, the crash state generator also provides a mode for
breaking these large operations into smaller sectors storage devices use. In
this mode, the algorithm uses the same two-step process described above to
generate crash states, but, instead of picking a subset of operations in the
target epoch, it picks a subset of the sectors that make up the operations in
the target epoch. While this gives a slightly more realistic view of the crash
state, it may not perfectly emulate device behavior for hard drives because it
has no logic to capture the fact that disk sectors are often written
sequentially. Sequential persistence of sectors means that it is unlikely that
the hard drive will drop some sectors in the middle of a contiguous range of
sectors. However, given the right sector size, the crash state generator may
reasonably emulate SSDs and NVMe where Flash Translation Layers (FTLs) are used
internally to remap logical sector numbers to different parts of the disk for
wear-leveling. A further study of how newer devices like SSDs and NVMe use FTLs
and the default sector size of these devices could lead to more realistic
behavior when using the crash state generator in this mode.

\am{NVMe has FTLs right? I haven't read all that much about them, so I'm not
sure if that is a correct statement :) I am just assuming internally they work
like SSDs with a different comunication protocol}

\subsection{Automating \sysnamet}
\label{sec-explore}

\vheading{Generating Workloads}.
\jm{Do we want to have this section here? I think \usysname talks about this in detail.
We could talk only about auto check here. }

\am{we may want to modify the below paragraph to say we do deeper comparisons
with the oracle disk image than just checking the fsynced file. For example, the
btrfs bug where renames of directories may not be persisted cause files to
appear at paths that weren't fsynced, but having those files present is a bug
since the user never created a file at that path}

\vheading{Generating Correctness Checks}. Automatic correctness tests need to
ensure the metadata and data in files referenced by operations like \sysfsync is
correct. Since checking the metadata and data of files for arbitrary sequences
of file system operations, of which only a subset may have completed, is hard,
\lsysname currently supports automatic correctness checks on crash states
generated by replaying to each \chkpt mark in the profiled workload. Reducing
the crash state space in this way allows \lsysname to use the disk snapshots
made at each \chkpt call in the workload as oracles which it can query to
determine the correct state of the disk in the crash state. Since each disk
snapshot represents the state of the disk after a different call to \chkpt, all
the automatic tester needs to operate is a generated crash state, the disk
snapshot that corresponds to the \chkpt mark that crash state is generated at,
and a list of the file that were affected by the file system operation that
created the persistence point. For example, if the persistence point was created
by a call to \sysfsync, then the auto tester only needs to query the oracle disk
image about the file or directory that the \sysfsync was called on. On the other
hand, if the operation that created the persistence point was a \sync operation,
then all of the contents on the generated crash state should match the contents
of the oracle disk image.

\vheading{Analyzing bug reports}. At each \chkpt, the autochecker compares the disk 
contents with the oracle to determine any inconsistencies and a diff-file is generated if 
there is a mismatch. We analyze the bug reports in two stages.

First, we run workloads in increasing order of sequence numbers. If a workload reports 
failure in sequence length 1, an ideal scenario is to patch the bug and then run 
sequence higher sequences, else the sequence 1 bug can show up in higher 
sequences, thereby producing the same bug reports as known bugs. Since the 
filesystem developers are typically slow on patching the reported bugs, to ensure the 
bugs we report are unique, we run \ftrace to ensure the codepaths are different.

Second, the way our workloads are generated helps us post-process the bug reports 
without requiring much manual effort. We classify workloads by the core sequence of 
operations in them - irrespective of the type of persistence points inserted into them. It 
is highly unlikely that the same set of operations lead to different bugs just by the 
change of persistence operations. For all the workloads in such a classified set, we only 
record the unique errors reported; if two workloads from the same set report the same 
error, then the bugs must be identical. This approach reduce the manual effort involved 
in investigating bug reports - as we have only 1 bug report for every unique 
combination of the core sequence. Starting with a set of 14 system calls, we investigate 
14 reports for workloads of sequence 1 and 196 reports for sequence length 2. Since 
we run sequence 3 on a constrained set of 5 system calls, we investigate only 125 bug 
reports. 





==> fig-bkgd.tex <==
\begin{figure}[!t]
  \centering \includegraphics[width=0.35\textwidth]{figures/bkgd-crop}
  \mycaption{Life of a file-system write}{The figure shows an
    application write being processed by the storage stack. For
    correctness, the data for the file needs to be persisted before
    the metadata. The file system sets the FLUSH flag when submitting
    the request to the block subsystem; the block subsystem flushes
    the data block before persisting the metadata block.}
  \label{fig-bkgd}
\end{figure}


==> limit.tex <==
\section{Limitations and Discussion}
\label{sec-limit}



==> tbl-crashtester.tex <==
\begin{table}[t]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}lr@{}}
    \toprule[1.2pt]
     Stages & \# Time taken (ms) \\
    \midrule
    \emph{Profiling the workload}\\
    Formatting and mounting the device &  100\\
    Mount delay & 1000\\
    Insert kernel modules & 378\\
    Snapshot & 56\\
    Writeback delay & 2000\\
    Unmounting the device & 7\\
    \emph{Sub Total} & 3541\\
    
    \midrule
    \emph{Constructing a crash state} & 21\\
    
    \midrule
    \emph{Testing consistency}\\
    Mounting disks & 1009\\
    Read checks & 16\\
    Write checks & 3\\
    \emph{Sub Total} & 1028 \\
    \midrule
    Total &  4590\\
    \bottomrule[1.2pt]
  \end{tabular}
  \vspace{-3pt}
  \mycaption{\lsys Performance}{The table shows the time spent in each
    stage of \lsys. The end-to-end latency to output the bug report is
    4.6 seconds.}
  \label{tbl-crashtester}
  \vspace{-5pt}
\end{table}


==> tbl-file-ops.tex <==
\begin{table*}[!t]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}llll@{}}
    \toprule[1.2pt]
    \seqone and \seqtwo  & \mseqthree &  \dseqthree & \nseqthree\\
    \midrule
    \texttt{creat, mkdir, falloc, buffered write, direct-IO write, mmap, link, unlink, rmdir,
setxattr, removexattr, remove, unlink} and 
\texttt{truncate}. 
 & Small workloads of 2-3 core operations & Maximum \# core ops in a workload is \emph{three} & hello \\
    \bottomrule[1.2pt]
  \end{tabular}
  \vspace{-5pt}  
  \mycaption{System calls tested in different workload sequences}{The table shows the list of filesystem operations that were tested in each of the workload sequence categories. \seqone and \seqtwo test the entire set of 14 system calls, while \seqthree focuses on a smaller set of operations due to the limited computation budget and the large number of workloads to be tested.}
  \label{tbl-file-ops}
\vspace{-0.1in}  
\end{table*}


==> tbl-newbugs.tex <==
\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}lr@{}}
    \toprule[1.2pt]
    File System & \# bugs \\
    \midrule
    btrfs & 6 \\
    F2FS & 2 \\
    \midrule
    Total & 8 \\
    \bottomrule[1.2pt]
  \end{tabular}
  \hfill
  \begin{tabular}{@{}lr@{}}
    \toprule[1.2pt]
    \# of ops required & \# bugs \\
    \midrule
    1 & 3 \\
    2 & 3 \\
    3 & 2 \\
    \midrule
    Total & 8 \\
    \bottomrule[1.2pt]
  \end{tabular}

  \mycaption{Analyzing New Crash-Consistency Bugs}{The tables breakdown
    the 8 new crash-consistency bugs reported by \sysname by filesystem and the
    number of operations required to reveal the bug. All these bugs appear on
    the most recent stable kernel - 4.16 - and their consequence is file-system corruption.}
  
  \label{tbl-newbugs}
\end{table}


==> tbl-workloads-per-seq.tex <==
\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}lc@{}R{3cm}@{}}
    \toprule[1.2pt]
    Sequence length& \# workloads& Running time (minutes) \\
    \midrule
    seq-1 & 300 & 1\\
    seq-2 & 254K & 215 \\
    seq-3-data & 120K & 102 \\
    seq-3-metadata & 1.5M & 1274\\
    seq-3-nested & 1.5M & 1274\\
    \midrule
    Total & 3.37M & 2866 \\
    \bottomrule[1.2pt]
  \end{tabular}
  
  \mycaption{Workloads tested}{The table shows the number of workloads
    tested in each set, along with the time taken to test these
    workloads in parallel on 65 physical machines. Overall, we tested
    3.37 million workloads in two days, reproducing 24 known bugs and
    finding 10 new crash-consistency bugs.}
  \label{tbl-workloads-per-seq}
\end{table}


==> tbl-workloads-setup.tex <==
\begin{table}[t]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}lr@{}}
    \toprule[1.2pt]
    Overhead & \# Time taken (min) \\
    \midrule
    Workload Generation & 374 \\
    Grouping by virtual machines & 34 \\
    Copy to nodes &  199\\
    Copy to virtual machines & 4 \\
    \midrule
    Total & 611 \\
    \bottomrule[1.2pt]
  \end{tabular}
  \mycaption{Time taken in setting up workloads on the Chameleon
    cloud}{The table breaks down the time taken by a single server to
    prepare workloads to be run on the 65-node Chameleon cluster.}
  \label{tbl-workloads-setup}
\end{table}

